Peacock: A Family of Arabic Multimodal Large Language Models and Benchmarks

Multimodal large language models (MLLMs) have proven effective in a wide range of tasks requiring complex reasoning and linguistic comprehension. However, due to a lack of high-quality multimodal resources in languages other than English, success of MLLMs remains relatively limited to English-based settings. This poses significant challenges in developing comparable models for other languages, including even those with large speaker populations such as Arabic. To alleviate this challenge, we introduce a comprehensive family of Arabic MLLMs, dubbed \textit{Peacock}, with strong vision and language capabilities. Through comprehensive qualitative and quantitative analysis, we demonstrate the solid performance of our models on various visual reasoning tasks and further show their emerging dialectal potential. Additionally, we introduce ~\textit{Henna}, a new benchmark specifically designed for assessing MLLMs on aspects related to Arabic culture, setting the first stone for culturally-aware Arabic MLLMs.The GitHub repository for the \textit{Peacock} project is available at \url{https://github.com/UBC-NLP/peacock}.

==> sections/model_archs.tex <==


\section{Lavender Models}

The overall architecture of the Lavender-VL series consists of three components: Vision encoder, Vision Language connector, and Large Language model (LLM). Below, we describe the two different models and their respective architectures. 

\subsection{Lavender-VL-Base}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{figs/pdfresizer.com-pdf-crop (2).pdf}
\centering
\caption{Illustration of the Lavender-VL-Base} \label{fig:vl-base}
\end{figure}

\paragraph{Vision encoder:}
We adopt Vision Transformer (ViT)~\cite{dosovitskiy2021image} as the visual encoder to extract a fixed number of output features from the images, initialized with pre-trained weights from ViT/G-14~\citep{fang2022eva}. 
We remove the last layer of the ViT and use the second last layer’s output features, which leads to slightly better performance. The Vision encoder is 1.1B in model parameters. 

\paragraph{Vision Language connector:}

In Lavender-VL-Base, the Q-Former, based on the model from InstructBlip~\citet{li2023blip, dai2023instructblip}, bridges the gap between the pretrained image encoder and the Large Language Model (LLM). The Q-Former comprises two transformer submodules with shared self-attention layers: firstly, an image transformer compressing image features from 256×768 to 64, using learnable visual query embeddings and self-attention layers. Secondly, a text transformer that encodes text presentations with input images. This setup enables the alignment of vision-language features by controlling query-text visibility using a self-attention mask matrix, facilitating various pre-training tasks. In the instruction-tuning phase, the model feeds the compressed visual feature sequence into the LLM.

\paragraph{Large Language model (LLM):}
In this approach, state-of-the-art (SOTA) Arabic Large Language Models (LLMs) such as AceGPT~\citet{huang2023acegpt}, $AraT5_{v2}$~\citet{elmadany2023octopus}, and the superior \jasmine model are utilized to construct the Lavender-VL-Base. The strategy is based on the observation that higher-performing LLMs contribute to developing more effective Vision Language Models (VLMs). Therefore, only the best Arabic LLMs are selected for this purpose. The LLM in this model architecture processes visual and textual inputs by concatenating them, leading to the generation of the final output. This methodology underscores the importance of choosing top-performing LLMs to enhance VLM capabilities.

\subsection{Lavender-VL-chat}

\begin{figure}[ht]
\includegraphics[width=\columnwidth]{figs/pdfresizer.com-pdf-crop (3).pdf}
\centering
\caption{Illustration of the Lavender-VL-Chat} \label{fig:vl-chat}
\end{figure}

\paragraph{Vision encoder:}

We use CLIP-VIT-L/14 as the vision encoder. CLIP~\citet{radford2021learning} combines a vision encoder (usually a Vision Transformer) and a language encoder (transformer-based) to process images and text. It is trained on large image-text pair datasets using contrastive learning to match corresponding pairs and differentiate non-matching ones. This architecture enables effective understanding and association of visual and textual information.

\paragraph{Vision Language connector:}
Drawing on advancements in self-supervised learning that demonstrate the benefits of transitioning from linear projection to a multilayer perceptron (MLP)~\cite{chen2020simple, mocov2}. By replacing the traditional linear projection with a two-layer MLP in the vision-language connector, we improve the model's multimodal processing abilities, reflecting the increased representational power of this approach.

\paragraph{Large Language model (LLM):}

For Lavender-VL-Chat, we continue to leverage state-of-the-art Arabic Large Language Models (LLMs), consistent with the approach in Lavender-VL-Base. The utilization of advanced LLMs like AceGPT, and \jasmine remains central to our strategy, given their proven efficacy in enhancing Vision Language Models (VLMs). In Lavender-VL-Chat, these high-performing LLMs are specifically tailored to support more interactive and conversational contexts, aligning with the model's focus on chat-based applications. The LLM in Lavender-VL-Chat adeptly handles concatenated visual and textual inputs, efficiently generating contextually relevant and conversationally coherent outputs. This adaptation underlines top-tier LLMs' versatility in improving VLM capabilities and fitting diverse application scenarios, especially in dialogue-based interactions.

==> tables/egy_results.tex <==
\begin{table}[t]

\centering



\scalebox{0.55}{
\begin{tabular}{@{}ll|cc}
\toprule
   Architecture&  LLM& XXX& YYY\\ \midrule
 \rowcolor{green!10} InstructBlip& AceGPT& xx.xx&yy.yy\\ 
  \rowcolor{blue!10} InstructBlip&   $Jasmine_{v2}$& xx.xx& yy.yy\\
          \bottomrule
\end{tabular}
}

\caption{Evaluation of InstructBlip-\jasmine and InstructBlip-AceGPT models on Egyption Dailect.}
\label{tab:egy_dialect_result}
\end{table}

==> tables/tasks.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begin{tabular}{lrrrrr}\toprule
\textbf{TASK} &\textbf{Name} &\textbf{Train} &\textbf{Val} &\textbf{Test} \\\midrule
\multirow{3}{*}{Caption} &COCO &566,747 &25,010 &25,010 \\
% &CCM3 &2.7M &- &- \\
&Flickr8K &6k &1k &1k \\
&xm3600 &- &- &7600 \\\hline
Reasoning &Winoground &- &- &800 \\\hline
\multirow{5}{*}{VQA} &VQAv2 &443,757 &214,354 &447,793 \\
&GVQ &943000 &132062 &12578 \\
&Visual7W &28653 &- &- \\
&VizWiz &10.3k &4.32k &8k \\
&OK-VQA &9k &5.05k &- \\\hline
Image Classifcation &Imagenet &30,000 &50,000 &- \\
\bottomrule
\end{tabular}
\caption{Table for all tasks}\label{tab: tasks}
\end{table}
